Activity Identification and Local Linear Convergence of Douglas--Rachford/ADMM under Partial Smoothness

Convex optimization has become ubiquitous in most quantitative disciplines of science, including variational image processing. Proximal splitting algorithms are becoming popular to solve such structured convex optimization problems. Within this class of algorithms, Douglas--Rachford (DR) and alternating direction method of multipliers (ADMM) are designed to minimize the sum of two proper lower semi-continuous convex functions whose proximity operators are easy to compute. The goal of this work is to understand the local convergence behaviour of DR (resp. ADMM) when the involved functions (resp. their Legendre-Fenchel conjugates) are moreover partly smooth. More precisely, when both of the two functions (resp. their conjugates) are partly smooth relative to their respective manifolds, we show that DR (resp. ADMM) identifies these manifolds in finite time. Moreover, when these manifolds are affine or linear, we prove that DR/ADMM is locally linearly convergent. When $J$ and $G$ are locally polyhedral, we show that the optimal convergence radius is given in terms of the cosine of the Friedrichs angle between the tangent spaces of the identified manifolds. This is illustrated by several concrete examples and supported by numerical experiments.

==> tex/sec-alternative.tex <==
\section{An Alternative}



\subsection{Primal DR}

For simplicity, let $\lambda_k \equiv 1$,
\begin{equation}
\left\{
\begin{aligned}
\vkp &= \prox_{\gamma G}\pa{2\xk - \zk}  , \\
\zkp &= \zk + \vkp - \xk  , \\
\xkp &= \prox_{\gamma J} \zkp  ,
\end{aligned}
\right.
~\Longleftrightarrow~
\left\{
\begin{aligned}
\pa{2\xk - \zk} - \vkp &\in \gamma \partial G\pa{\vkp}  , \\
\zkp &= \zk + \vkp - \xk  , \\
\zkp - \xkp &\in \gamma\partial J(\xkp)   .
\end{aligned}
\right.
\end{equation}
There exists $p^{k+1} \in \partial G(\vkp)$ and $q^{k+1} \in \partial J(\xkp)$, such that
\[
\begin{aligned}
\vkp = \pa{2\xk - \zk} - \gamma p^{k+1}  &,~~~  
\xkp = \zkp - \gamma q^{k+1}  , \\
\vsol = \pa{2\xsol - \zsol} - \gamma p^{\star}  &,~~~  
\xsol = \zsol - \gamma q^{\star}  .
\end{aligned}
\]
% 
We have
\[
\begin{aligned}
\xk-\xsol 
&= \PJ(\xk-\xsol) 
= \PJ\Pa{(\zk-\gamma q^{k}) - (\zsol-\gamma q^\star)}  \\
&= \PJ\pa{\zk-\zsol} - \gamma \pa{e_J^{k} - e_J^\star} ,  \\
% 
\vkp-\xsol 
&= \PG(\vkp-\xsol)  \\
&= \PG\Pa{(2\xk-\zk-\gamma p^{k+1}) - (2\xsol-\zsol-\gamma p^{\star})}  \\
&= 2\PG(\xk-\xsol) - \PG(\zk-\zsol) - \gamma\pa{e_G^{k+1} - e_G^{\star}}  \\
&= 2\PG\Pa{\PJ\pa{\zk-\zsol} - \gamma \PJ\pa{q^k - q^\star}} - \PG(\zk-\zsol) - \gamma\pa{e_G^{k+1} - e_G^{\star}}  \\
&= 2\PG\PJ\pa{\zk-\zsol} - 2\gamma \PG\pa{e_J^k - e_J^\star} - \PG(\zk-\zsol) - \gamma\pa{e_G^{k+1} - e_G^{\star}}  \\
&= \Pa{2\PG\PJ - \PG}\pa{\zk-\zsol} - 2\gamma \PG\pa{e_J^k - e_J^\star} - \gamma\pa{e_G^{k+1} - e_G^{\star}}  .
\end{aligned}
\]
Then
\[
\begin{aligned}
& \pa{\zk+\vkp-\xk} - \zsol  \\
=~& \pa{\zk+\vkp-\xk} - \pa{\zsol+\xsol-\xsol} \\
=~& \pa{\zk-\zsol} + \pa{\vkp-\xsol} - \pa{\xk-\xsol} \\
=~& \Pa{\Id + 2\PG\PJ - \PG - \PJ}\pa{\zk-\zsol} - \gamma \PJ\pa{q^k - q^\star}  \\ \qquad& - 2\gamma \PG\PJ\pa{q^k - q^\star} - \gamma\pa{e_G^{k+1} - e_G^{\star}}   
\end{aligned}
\]


%%%%%%%%%%%%%%%%%%%
\subsubsection{$J$ is locally polyhedral}
There exists $p^{k+1} \in \partial G(\vkp)$ and $q^{k+1} \in \partial J(\xkp)$, such that
\[
\begin{aligned}
\vkp = \pa{2\xk - \zk} - \gamma p^{k+1}  &,~~~  
\xkp = \zkp - \gamma q^{k+1}  , \\
\vsol = \pa{2\xsol - \zsol} - \gamma p^{\star}  &,~~~  
\xsol = \zsol - \gamma q^{\star}  .
\end{aligned}
\]
\[
\begin{aligned}
\xk-\xsol 
&= \PJ(\xk-\xsol) 
= \PJ\Pa{(\zk-\gamma q^{k}) - (\zsol-\gamma q^\star)}  
= \PJ\pa{\zk-\zsol} ,  \\
% 
\vkp-\xsol 
&= \PG(\vkp-\xsol) 
= \PG\Pa{(2\xk-\zk-\gamma p^{k+1}) - (2\xsol-\zsol-\gamma p^{\star})}  \\
&= 2\PG(\xk-\xsol) - \PG(\zk-\zsol) - \gamma\pa{e_G^{k+1} - e_G^{\star}}  \\
&= 2\PG\PJ\pa{\zk-\zsol} - \PG(\zk-\zsol) - \gamma\pa{e_G^{k+1} - e_G^{\star}}  \\
&= \Pa{2\PG\PJ - \PG}\pa{\zk-\zsol} - \gamma\pa{e_G^{k+1} - e_G^{\star}}  .
\end{aligned}
\]
Then
\[
\begin{aligned}
\zkp - \zsol 
&= \pa{\zk+\vkp-\xk} - \zsol  \\
&= \pa{\zk+\vkp-\xk} - \pa{\zsol+\xsol-\xsol} \\
&= \pa{\zk-\zsol} + \pa{\vkp-\xsol} - \pa{\xk-\xsol} \\
&= \Pa{\Id + 2\PG\PJ - \PG - \PJ}\pa{\zk-\zsol} - \gamma\pa{e_G^{k+1} - e_G^{\star}}  .
\end{aligned}
\]
With $\gamma p^{k+1} = \pa{2\xk - \zk} - \vkp = \xk - \zkp$, we have
\[
\begin{aligned}
\gamma^2\norm{e_G^{k+1} - e_G^{\star}}^2
&= \iprod{\pa{\xk - \zkp}-\pa{\xsol - \zsol}}{\pa{\xk - \zkp}-\pa{\xsol - \zsol}}_{\PG}  \\
&= \norm{\xk-\xsol}_{\PG}^2 + \norm{\zkp-\zsol}_{\PG}^2 + 2\iprod{\xk - \xsol}{\zkp - \zsol}_{\PG}  \\
%
2\gamma \iprod{\zkp - \zsol}{e_G^{k+1} - e_G^{\star}}
&= 2 \iprod{\zkp - \zsol}{\pa{\xk - \zkp}-\pa{\xsol - \zsol}}_{\PG}  \\
&= -2 \norm{\zkp - \zsol}^2_{\PG} - 2 \iprod{\zkp - \zsol}{\xk - \xsol}_{\PG}  .
\end{aligned}
\]
Then
\[
\begin{aligned}
\norm{\pa{\zkp - \zsol} + \gamma\pa{e_G^{k+1} - e_G^{\star}}}^2
&= \norm{\zkp - \zsol}^2 + \gamma^2\norm{e_G^{k+1} - e_G^{\star}}^2 + 2\gamma \iprod{\zkp - \zsol}{e_G^{k+1} - e_G^{\star}}  \\
&= \norm{\zkp - \zsol}^2 + \norm{\xk-\xsol}_{\PG}^2 - \norm{\zkp-\zsol}_{\PG}^2  .
\end{aligned}
\]
 If
\[
\begin{aligned}
\norm{\zkp-\zsol}_{\PG}^2 - \norm{\xk-\xsol}_{\PG}^2
&= o(\norm{\zkp-\zsol}^2)  ~~or~~ < 0 ?
\end{aligned}
\]


%%%%%%%%%%%%%%%%%%%
\subsection{Primal--Dual setting}
The key idea to understand the finite identification property of DR is to look at its primal-dual formulation. More precisely, one can easily check that \eqref{eq:drsgen} is equivalent to
\begin{equation}\label{eq:drsprimaldual}
\left\{
\begin{aligned}
\ukp &= \prox_{G^*/\gamma}\Pa{\pa{2 \xk - \zk}/{\gamma}}  , \\
\zkp &= (1-\lambda_k)\zk + \lambda_k \pa{\xk - \gamma \ukp} ,  \\
\xkp &= \prox_{\gamma J}\pa{\zkp}  . \\
\end{aligned}
\right. 
\end{equation}
The sequence $\uk$ can be interpreted as the iterates of a dual variable $u$.

It is worth mentioning that when $\lambda_k \equiv 1$, by virtue of Moreau identity, \eqref{eq:drsprimaldual} becomes the primal-dual relaxed Arrow-Hurwicz scheme \cite{chambolle2011first}
\begin{equation*}
\left\{
\begin{aligned}
\ukp &= \prox_{G^*/\gamma}\pa{\uk + \bar{x}^k/\gamma}   , \\
\xkp &= \prox_{\gamma J}\pa{\xk - \gamma \ukp}  , \\
\bar{x}^{k+1} &= 2 \xkp - \xk  ,
\end{aligned}
\right.
\end{equation*}
where $\bar{x}^{k} = 2 \xk - \xkm$ and $\zk = \xkm - \gamma \uk$.

We have, denote $\tau = 1/\gamma$
\begin{equation*}
\left\{
\begin{aligned}
\ukp &= \prox_{\tau G^*}\pa{\uk + \tau \bar{x}^k}   , \\
\xkp &= \prox_{\gamma J}\pa{\xk - \gamma \ukp}  , \\
\bar{x}^{k+1} &= 2 \xkp - \xk  ,
\end{aligned}
\right.
~\Longleftrightarrow~
\left\{
\begin{aligned}
\pa{\uk + \tau\bar{x}^k} - \ukp &\in \tau \partial {G^*}\pa{\ukp}   , \\
\pa{\xk - \gamma \ukp} - \xkp &\in \gamma \partial{J}\pa{\xkp}  , \\
\bar{x}^{k+1} &= 2 \xkp - \xk  ,
\end{aligned}
\right.
\end{equation*}

Since $J$ is locally polyhedral,
\[
\begin{aligned}
\pa{\bar{x}^k - \xsol} 
&= \PJ\Pa{(2\xk-\xkm) - \xsol} \\
&= 2\PJ(\xk-\xsol) - \PJ(\xkm-\xsol) \\
&= \PJ\pa{\xkm - \xsol} - 2\gamma \PJ\pa{\uk - \usol}  ,
\end{aligned}
\]
for $\uk-\usol$, we have
\[
\uk-\usol
= \PGc\pa{\uk-\usol} + o\pa{\norm{\uk-\usol}}   ,
\]
then by virtue of the non-expansiveness of the proximity operator, we have
\[
\begin{aligned}
\gamma\norm{\ukp-\usol} 
&\leq \norm{\pa{\gamma\uk + \bar{x}^k} - \pa{\gamma\usol + \xsol}}  
= \norm{\gamma\pa{\uk - \usol} + \pa{\bar{x}^k - \xsol}}  \\
&= \norm{\pa{\Id-2\PJ}\PGc\gamma\pa{\uk-\usol} + \PJ\pa{\xkm-\xsol} + o\pa{\norm{\uk-\usol}}}  \\
&\leq \norm{\pa{\Id-2\PJ}\PGc\gamma\pa{\uk-\usol} + \PJ\pa{\xkm-\xsol}} + o\pa{\norm{\uk-\usol}}  ,
\end{aligned}
\]
and 
\[
\begin{aligned}
\norm{\xk-\xsol}
&= \norm{\PJ\pa{\xkm - \xsol} - \gamma \PJ\PGc\pa{\uk - \usol} + o\pa{\norm{\uk-\usol}}}  \\
&\leq \norm{\PJ\pa{\xkm - \xsol} - \gamma \PJ\PGc\pa{\uk - \usol}} + o\pa{\norm{\uk-\usol}}   ,
\end{aligned}
\]
therefore, we can derive that
\[
\begin{aligned}
\begin{Vmatrix} \gamma\pa{\ukp-\usol} \\ \xk-\xsol \end{Vmatrix}^2
&\leq 
\begin{Vmatrix} 
\begin{bmatrix}
\pa{\Id-2\PJ}\PGc  & \PJ  \\ -\PJ\PGc & \PJ
\end{bmatrix}
\begin{pmatrix}
\gamma\pa{\uk-\usol} \\ \xkm-\xsol
\end{pmatrix}
\end{Vmatrix}^2
+ o\Ppa{\begin{Vmatrix}{\begin{pmatrix}
\gamma\pa{\uk-\usol} \\ \xkm-\xsol
\end{pmatrix}}\end{Vmatrix}^2}
\end{aligned}
\]

Suppose $\dim\pa{\TJ{\xsol}} = a, \dim\pa{T_{\usol}^{G^*}} = b$, and $a \leq b$.
\paragraph{Case 1, $a+b<n$:}
Then there exists an orthogonal matrix $D$ such that
\[
\PJ
= D\begin{bmatrix}
\Id_a & 0 & 0 & 0  \\
0 & 0_a & 0 & 0  \\
0 & 0 & 0_{b-a} & 0  \\
0 & 0 & 0 & 0_{n-a-b}  \\
\end{bmatrix} D^* ,~~
\PGc
= D\begin{bmatrix}
C^2 & CS & 0 & 0  \\
CS & S^2 & 0 & 0  \\
0 & 0 & \Id_{b-a} & 0  \\
0 & 0 & 0 & 0_{n-a-b}  \\
\end{bmatrix} D^*.
\]
Then
\[
\PJ\PGc
= D\begin{bmatrix}
C^2 & CS & 0 & 0  \\
0 & 0_a & 0 & 0  \\
0 & 0 & 0_{b-a} & 0  \\
0 & 0 & 0 & 0_{n-a-b}  \\
\end{bmatrix} D^* ,~~
\PGc\PJ
= D\begin{bmatrix}
C^2 & 0 & 0 & 0  \\
CS & 0_a & 0 & 0  \\
0 & 0 & 0_{b-a} & 0  \\
0 & 0 & 0 & 0_{n-a-b}  \\
\end{bmatrix} D^* .
\]
Denote $\proj_{} = \PGc - 2\PJ\PGc$,
\[
\abs{M-\rho\Id} 
= \begin{vmatrix}
	\begin{bmatrix}
		\proj_{} - \rho\Id_n & \PJ  \\
		-\PJ\PGc & \PJ-\rho\Id_n
	\end{bmatrix}
\end{vmatrix}  ,
\]
since $\PJ\pa{\PJ-\rho\Id_n} = \pa{\PJ-\rho\Id_n}\PJ$ \cite[Theorem 3]{silvester2000determinants}, then
\[
\begin{aligned}
\abs{M-\rho\Id} 
&= \begin{vmatrix}
	\begin{bmatrix}
		\proj_{} - \rho\Id_n & \PJ  \\
		-\PJ\PGc & \PJ-\rho\Id_n
	\end{bmatrix}
\end{vmatrix}  \\
&= \begin{vmatrix}
	\begin{bmatrix}
		\Pa{\PJ-\rho\Id_n}\Pa{\proj_{} - \rho\Id_n} + \PJ\PGc 
	\end{bmatrix}
\end{vmatrix}  \\
&= \begin{vmatrix}
	\begin{bmatrix}
		\rho^2\Id_n - \rho\pa{\PJ+\PGc-2\PJ\PGc} 
	\end{bmatrix}
\end{vmatrix}  \\
%&= \begin{vmatrix}
%	\begin{bmatrix}
%	\rho^2\Id_a & 0 & 0 & 0 \\  0 & \rho^2\Id_a & 0 & 0 \\  0 & 0 & \rho^2\Id_a & 0 \\  0 & 0 & 0 & \rho^2\Id_a
%	\end{bmatrix}
%	- \rho
%	\begin{bmatrix}
%	\Id_a-C^2 & -CS & 0 & 0  \\
%        CS & S^2 & 0 & 0  \\
%        0 & 0 & \Id_{b-a} & 0  \\
%        0 & 0 & 0 & 0_{n-a-b}  \\
%	\end{bmatrix}
%\end{vmatrix}  \\
&= \begin{vmatrix}
	\begin{bmatrix}
	\rho^2\Id_a-\rho S^2 & \rho CS & 0 & 0 \\  -\rho CS & \rho^2\Id_a - \rho S^2 & 0 & 0 \\  0 & 0 & \rho\pa{\rho-1}\Id_{b-a} & 0 \\  0 & 0 & 0 & \rho^2\Id_{n-a-b}
	\end{bmatrix}
\end{vmatrix}  \\
&= \rho^{2n-3a-b}\pa{\rho-1}^{b-a} \begin{vmatrix}
	\begin{bmatrix}
	\rho^2\Id_a-\rho S^2 & \rho CS  \\  -\rho CS & \rho^2\Id_a - \rho S^2 
	\end{bmatrix}
\end{vmatrix}  \\
%&= \rho^{2n-3a-b}\pa{\rho-1}^{b-a} \begin{vmatrix} \pa{\rho^2\Id_a-\rho S^2}^2 + \rho^2 C^2S^2 \end{vmatrix}  \\
%&= \rho^{2n-3a-b}\pa{\rho-1}^{b-a} \rho^{2a} \begin{vmatrix} \pa{\rho\Id_a - S^2}^2 + C^2S^2 \end{vmatrix}  \\
%&= \rho^{2n-a-b}\pa{\rho-1}^{b-a} \begin{vmatrix} \rho^2\Id_a -2\rho S^2 + S^2 \end{vmatrix}  \\
&= \rho^{2n-a-b}\pa{\rho-1}^{b-a} \prod_{j=1}^a \Pa{ \rho^2 - 2\rho S_j^2 + S_j^2 }  .
\end{aligned}
\]
Hence we get, besides $0$ and $1$,
\[
\rho_j = S_j^2 \pm i C_jS_j   ~~~\mathrm{and}~~~ \abs{\rho_j} = S_j  .
\]
For the eigenvalues equal to $1$, we have
\[
{M-\Id} 
= \begin{bmatrix}
	C^2 & CS & 0 & 0 \\  - CS & C^2 & 0 & 0 \\  0 & 0 & 0_{b-a} & 0 \\  0 & 0 & 0 & \Id_{n-a-b}
	\end{bmatrix}  ,~
\pa{M-\Id}^2 
= \begin{bmatrix}
	C^4-C^2S^2 & 2C^3S & 0 & 0 \\  - 2C^3S & C^4-C^2S^2 & 0 & 0 \\  0 & 0 & 0_{b-a} & 0 \\  0 & 0 & 0 & \Id_{n-a-b}
	\end{bmatrix}  ,
\]
it is easy to check that $\rank(M-\Id) = \rank\Pa{(M-\Id)^2}=2n+a-b$, hence eigenvalue $1$ is semisimple \cite[Fact 2.3]{Bauschke14}. Then, owing to \cite[Theorem 2.12]{Bauschke14}, we have $M$ is convergent with rate $\max(S)$.
Namely, the rate is the sine of the largest Friedrichs angle (smaller than $\pi/2$), which is the supplementary angle of the smallest Friedrichs angle (bigger than $0$) between $T_{\xsol}^J$ and $T_{\vsol}^G$ when $G$ is also locally polyhedral.


\paragraph{Case 2, $a+b \geq n$:}
For this case, applying the dimension enlargement trick \cite[Section 3]{Bauschke14} leads to the desired result.

%%%%%%%%%%%%%
%\subsubsection{. .. ... ....}
%
%There exists $p^{k+1} \in \partial G^*(\ukp)$ and $q^{k} \in \partial J(\xk)$, such that
%\[
%\begin{aligned}
%\ukp = \pa{\uk + \tau\bar{x}^k} - \tau p^{k+1}  &,~~~  
%\xk = \pa{\xkm - \gamma \uk} - \gamma q^{k}  , \\
%\usol = \pa{\usol + \tau \xsol} - \tau p^{\star}  &,~~~  
%\xsol = \pa{\xsol - \gamma \usol} - \gamma q^{\star}  .
%\end{aligned}
%\]
%$\Longrightarrow$
%\[
%\begin{aligned}
%\ukp - \usol &= \PGc(\ukp - \usol) = \PGc\Pa{\pa{\uk + \tau\bar{x}^k}-\pa{\usol + \tau \xsol}} - \tau(e_{G^*}^{k+1} - e_{G^*}^{\star})  \\ 
%\xk - \xsol &= \PJ(\xk - \xsol) = \PJ\Pa{\pa{\xkm - \gamma \uk}-\pa{\xsol - \gamma \usol}} - \gamma(e_J^{k}-e_J^\star) .
%\end{aligned}
%\]
%and
%\[
%\begin{aligned}
%& \begin{pmatrix}
%(\ukp - \usol) + \tau(e_{G^*}^{k+1} - e_{G^*}^{\star})  \\
%(\xk - \xsol) + \gamma(e_J^{k}-e_J^\star)  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\PGc\pa{\uk - \usol} + \tau \PGc\pa{\bar{x}^k - \xsol}  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\PGc\pa{\uk - \usol} + 2\tau \PGc\pa{\xk - \xsol} - \tau \PGc\pa{\xkm - \xsol}  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{bmatrix}
%\PGc & 2\tau \PGc & - \tau \PGc \\
%- \gamma \PJ & 0 & \PJ \\
%\end{bmatrix}
%\begin{pmatrix}
%{\uk - \usol} \\ 
%{\xk - \xsol} \\
%{\xkm - \xsol} 
%\end{pmatrix}.
%\end{aligned}
%\]
%
%% \newpage
%
%\subsubsection{$J$ is locally polyhedral}
%
%If $J$ is locally polyhedral, then
%\[
%\begin{aligned}
%\ukp - \usol 
%&= \PGc(\ukp - \usol) 
%% = \PGc\Pa{\pa{\uk + \tau\bar{x}^k}-\pa{\usol + \tau \xsol}} - \tau(e_{G^*}^{k+1} - e_{G^*}^{\star})
%= \PGc\pa{\uk - \usol} + \tau\PGc\PJ\pa{\bar{x}^k - \xsol} - \tau(e_{G^*}^{k+1} - e_{G^*}^{\star})  \\ 
%% 
%\xk - \xsol 
%&= \PJ(\xk - \xsol) 
%% = \PJ\Pa{\pa{\xkm - \gamma \uk}-\pa{\xsol - \gamma \usol}}
%= \PJ\pa{\xkm - \xsol} - \gamma \PJ\PGc\pa{\uk - \usol}  .
%\end{aligned}
%\]
%We have 
%\[
%\begin{aligned}
%\PGc\PJ\pa{\bar{x}^k - \xsol} 
%&= \PGc\PJ\Pa{(2\xk-\xkm) - \xsol} \\
%&= \PGc\PJ\Pa{2(\xk-\xsol) - (\xkm-\xsol)} \\
%&= 2\PGc\PJ(\xk-\xsol) - \PGc\PJ(\xkm-\xsol) \\
%&= 2\PGc\PJ\pa{\xkm - \xsol} - 2\gamma \PGc\PJ\pa{\uk - \usol} - \PGc\PJ(\xkm-\xsol)  \\
%&= \PGc\PJ\pa{\xkm - \xsol} - 2\gamma \PGc\PJ \pa{\uk - \usol}   ,
%\end{aligned}
%\]
%then
%\[
%\begin{aligned}
%& \begin{pmatrix}
%\gamma (\ukp - \usol) + (e_{G^*}^{k+1} - e_{G^*}^{\star})  \\
%\xk - \xsol  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\gamma \PGc\pa{\uk - \usol} + \PGc\pa{\bar{x}^k - \xsol}  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\PGc\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\gamma \PGc\pa{\uk - \usol} + \PGc\PJ\pa{\xkm - \xsol} - 2\gamma \PGc\PJ\pa{\uk - \usol}   \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\PGc\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\gamma \Pa{\PGc - 2\PGc\PJ}\pa{\uk - \usol} + \PGc\PJ \pa{\xkm - \xsol}  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\PGc\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{bmatrix}
%\PGc - 2\PGc\PJ & \PGc\PJ  \\
%- \PJ\PGc & \PJ \\
%\end{bmatrix}
%\begin{pmatrix}
%\gamma \pa{\uk - \usol} \\ 
%{\xkm - \xsol} 
%\end{pmatrix}.
%\end{aligned}
%\]
%Denote
%\[
%M = \begin{bmatrix}
%\PGc - 2\PGc\PJ & \PGc\PJ  \\
%- \PJ\PGc & \PJ 
%\end{bmatrix} ,
%\]
%and is not normal.
%then
%\[
%\begin{aligned}
%MM^T
%&= \begin{bmatrix}
%\PGc - 2\PGc\PJ & \PGc\PJ \\
%- \PJ\PGc & \PJ 
%\end{bmatrix} \begin{bmatrix}
%\PGc - 2\PJ\PGc & - \PGc\PJ  \\
%\PJ\PGc & \PJ 
%\end{bmatrix}  \\
%&=  \begin{bmatrix}
%\PGc + \PGc\PJ\PGc & \PGc\PJ  \\
%\PJ\PGc & \PJ 
%\end{bmatrix}   ,\\
%M^TM
%&= \begin{bmatrix}
%\PGc - 2\PJ\PGc & - \PJ  \\
%2\PJ\PGc - \PGc & \PJ 
%\end{bmatrix}  \begin{bmatrix}
%\PGc - 2\PGc\PJ & {2\PGc\PJ - \PGc} \\
%- \PJ & \PJ 
%\end{bmatrix}  \\
%&= \begin{bmatrix}
%\PGc + \PJ & -\PGc - \PJ  \\
%-\PGc - \PJ & \PGc + \PJ 
%\end{bmatrix}  .
%\end{aligned}
%\]
%$\Longrightarrow M$ is not normal.



%Suppose $\dim\Pa{\TJ{\xsol}} = a, \dim\Pa{T_{\usol}^{G^*}} = b$ and $a \leq b, a+b < n$, then there exists an orthogonal matrix $D$ such that
%\[
%\PJ
%= D\begin{bmatrix}
%\Id_a & 0 & 0 & 0  \\
%0 & 0_a & 0 & 0  \\
%0 & 0 & 0_{b-a} & 0  \\
%0 & 0 & 0 & 0_{n-a-b}  \\
%\end{bmatrix} D^* ,~~
%\PGc
%= D\begin{bmatrix}
%C^2 & CS & 0 & 0  \\
%CS & S^2 & 0 & 0  \\
%0 & 0 & \Id_{b-a} & 0  \\
%0 & 0 & 0 & 0_{n-a-b}  \\
%\end{bmatrix} D^*.
%\]
%Then
%\[
%\PJ\PGc
%= D\begin{bmatrix}
%C^2 & CS & 0 & 0  \\
%0 & 0_a & 0 & 0  \\
%0 & 0 & 0_{b-a} & 0  \\
%0 & 0 & 0 & 0_{n-a-b}  \\
%\end{bmatrix} D^* ,~~
%\PGc\PJ
%= D\begin{bmatrix}
%C^2 & 0 & 0 & 0  \\
%CS & 0_a & 0 & 0  \\
%0 & 0 & 0_{b-a} & 0  \\
%0 & 0 & 0 & 0_{n-a-b}  \\
%\end{bmatrix} D^* ,
%\]
%therefore
%\[
%M = 
%\begin{bmatrix}D & 0 \\ 0 & D\end{bmatrix}
%\begin{bmatrix}
%-C^2 & CS & 0 & 0 & C^2 & 0 & 0 & 0 \\
%-CS & S^2 & 0 & 0 & CS & 0_a & 0 & 0 \\
%0 & 0 & \Id_{b-a} & 0 & 0 & 0 & 0_{b-a} & 0 \\
%0 & 0 & 0 & 0_{n-a-b} & 0 & 0 & 0 & 0_{n-a-b} \\
%-C^2 & -CS & 0 & 0 & \Id_{a} & 0 & 0 & 0 \\
%0 & 0_a & 0 & 0 & 0 & 0_a & 0 & 0 \\
%0 & 0 & 0_{b-a} & 0 & 0 & 0 & 0_{b-a} & 0 \\
%0 & 0 & 0 & 0_{n-a-b} & 0 & 0 & 0 & 0_{n-a-b} 
%\end{bmatrix}
%\begin{bmatrix}D^* & 0 \\ 0 & D^*\end{bmatrix}
%\]
%and 
%\[
%{M-\rho\Id} = 
%\begin{bmatrix}D & 0 \\ 0 & D\end{bmatrix}
%\begin{bmatrix}
%-C^2-\rho & CS & 0 & 0 & C^2 & 0 & 0 & 0 \\
%-CS & S^2-\rho & 0 & 0 & CS & 0_a & 0 & 0 \\
%0 & 0 & \Id_{b-a}-\rho & 0 & 0 & 0 & 0_{b-a} & 0 \\
%0 & 0 & 0 & -\rho & 0 & 0 & 0 & 0_{n-a-b} \\
%-C^2 & -CS & 0 & 0 & \Id_{a}-\rho & 0 & 0 & 0 \\
%0 & 0_a & 0 & 0 & 0 & -\rho & 0 & 0 \\
%0 & 0 & 0_{b-a} & 0 & 0 & 0 & -\rho & 0 \\
%0 & 0 & 0 & 0_{n-a-b} & 0 & 0 & 0 & -\rho 
%\end{bmatrix}
%\begin{bmatrix}D^* & 0 \\ 0 & D^*\end{bmatrix}
%\]
%then
%\[
%\begin{aligned}
%\abs{M-\rho\Id}
%&= \begin{vmatrix}
%    \begin{bmatrix}
%    -\pa{C^2+\rho}\pa{\Id-\rho} & -\rho CS & 0 & 0  \\
%    -CS\pa{\Id-\rho} & -\rho\pa{S^2-\rho} & 0 & 0  \\
%    0 & 0 & -\rho\pa{\Id_{b-a}-\rho} & 0  \\
%    0 & 0 & 0 & \rho^2 
%    \end{bmatrix} - 
%    \begin{bmatrix}
%    -C^4 & -C^3S & 0 & 0 \\
%    -C^3S & -C^2S^2 & 0 & 0 \\
%    0 & 0 & 0_{b-a} & 0 \\
%    0 & 0 & 0 & 0_{n-a-b}  
%    \end{bmatrix}
%\end{vmatrix}  \\
%&= \begin{vmatrix}
%    \begin{bmatrix}
%    -\pa{C^2+\rho}\pa{1-\rho} + C^4 & -\rho CS+C^3S & 0 & 0  \\
%    -CS\pa{1-\rho}+C^3S & -\rho\pa{S^2-\rho}+C^2S^2 & 0 & 0  \\
%    0 & 0 & -\rho\pa{1-\rho} & 0  \\
%    0 & 0 & 0 & \rho^2 
%    \end{bmatrix}
%\end{vmatrix}  \\
%&= \rho^{2n-b-3a}\pa{1-\rho}^{b-a}  % \Pa{\rho\pa{1-\rho}}^{b-a} \rho^{2(n-a-b)} 
%\begin{vmatrix}
%    \begin{bmatrix}
%    -\pa{C^2+\rho}\pa{1-\rho} + C^4 & -\rho CS+C^3S  \\
%    -CS\pa{1-\rho}+C^3S & -\rho\pa{S^2-\rho}+C^2S^2  \\
%    \end{bmatrix}
%\end{vmatrix}  \\
%\end{aligned}
%\]
%
%
%
%\[
%\begin{aligned}
%\abs{M-\rho\Id} 
%&= \begin{vmatrix}
%	\begin{bmatrix}
%		\PGc - 2\PGc\PJ - \rho\Id_n & \PGc\PJ  \\
%		-\PJ\PGc & \PJ-\rho\Id_n
%	\end{bmatrix}
%\end{vmatrix}  \\
%&= \begin{vmatrix}
%	\begin{bmatrix}
%		\Pa{\PGc - 2\PGc\PJ - \rho\Id_n}\Pa{\PJ-\rho\Id_n} + \PGc\PJ\PJ\PGc 
%	\end{bmatrix}
%\end{vmatrix}  \\
%&= \begin{vmatrix}
%	\begin{bmatrix}
%		\PGc\PJ - \rho\PGc - 2\PGc\PJ + 2\rho\PGc\PJ - \rho\PJ+\rho^2\Id_n + \PGc\PJ\PGc 
%	\end{bmatrix}
%\end{vmatrix}  \\
%&= \begin{vmatrix}
%	\begin{bmatrix}
%		\pa{2\rho - 1}\PGc\PJ - \rho\Pa{\PGc + \PJ} +\rho^2\Id_n + \PGc\PJ\PGc 
%	\end{bmatrix}
%\end{vmatrix}  \\
%\end{aligned}
%\]
%
%%%%%%%%%%%%%%%%%%%%
%\subsection{$G^*$ is locally polyhedral}
%
%\em{Nope..}
%
%If $G^*$ is locally polyhedral, then
%\[
%\begin{aligned}
%\ukp - \usol 
%&= \PGc(\ukp - \usol) 
%% = \PGc\Pa{\pa{\uk + \tau\bar{x}^k}-\pa{\usol + \tau \xsol}}
%= \PGc\pa{\uk - \usol} + \tau \PGc\pa{\bar{x}^k - \xsol}  \\ 
%% 
%\xk - \xsol 
%&= \PJ(\xk - \xsol) 
%= \PJ\pa{\xkm - \xsol} - \gamma \PJ\pa{\uk - \usol} - \gamma(e_J^{k}-e_J^\star) .
%\end{aligned}
%\]
%For $\PGc\pa{\bar{x}^k - \xsol}$,
%\[
%\begin{aligned}
%& \PGc\pa{\bar{x}^k - \xsol}  \\
%=~& \PGc\Pa{(2\xk-\xkm) - \xsol} \\
%=~& \PGc\Pa{2(\xk-\xsol) - (\xkm-\xsol)} \\
%=~& 2\PGc(\xk-\xsol) - \PGc(\xkm-\xsol) \\
%=~& 2\PGc\PJ\pa{\xkm - \xsol} - 2\gamma \PGc\PJ\pa{\uk - \usol} - 2\gamma\PGc(e_J^{k}-e_J^\star) - \PGc(\xkm-\xsol)  ,
%\end{aligned}
%\]
%then
%\[
%\begin{aligned}
%& \begin{pmatrix}
%\gamma (\ukp - \usol)  \\
%(\xk - \xsol) + \gamma(e_J^{k}-e_J^\star)  \\
%\end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\gamma \PGc\pa{\uk - \usol} + \PGc\pa{\bar{x}^k - \xsol}  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%% =~&
%% \begin{pmatrix}
%% \gamma \PGc\pa{\uk - \usol} + 2\PGc\PJ\pa{\xkm - \xsol} - 2\gamma \PGc\PJ\pa{\uk - \usol} - 2\gamma\PGc(e_J^{k}-e_J^\star) - \PGc(\xkm-\xsol)  \\
%% \PJ\pa{\xkm -  \xsol} - \gamma \PJ\pa{\uk - \usol}  \\
%% \end{pmatrix}  \\
%=~&
%\begin{pmatrix}
%\gamma \Pa{\PGc - 2 \PGc\PJ}\pa{\uk - \usol} + \Pa{2\PGc\PJ - \PGc}\pa{\xkm - \xsol} - 2\gamma\PGc(e_J^{k}-e_J^\star)  \\
%\PJ\pa{\xkm -  \xsol} - \gamma \PJ\pa{\uk - \usol}  \\
%\end{pmatrix}  \\
%=~&
%\begin{bmatrix}
%\PGc - 2 \PGc\PJ & 2\PGc\PJ - \PGc \\
%- \PJ & \PJ \\
%\end{bmatrix}
%\begin{pmatrix}
%\gamma \pa{\uk - \usol} \\ 
%{\xkm - \xsol} 
%\end{pmatrix} 
%+ \begin{pmatrix}
% - 2\gamma\PGc(e_J^{k}-e_J^\star)  \\
%0
%\end{pmatrix} .
%\end{aligned}
%\]
%

\newpage
